Progressive Feature Self-reinforcement for Weakly Supervised Semantic Segmentation

Compared to conventional semantic segmentation with pixel-level supervision, Weakly Supervised Semantic Segmentation (WSSS) with image-level labels poses the challenge that it always focuses on the most discriminative regions, resulting in a disparity between fully supervised conditions. A typical manifestation is the diminished precision on the object boundaries, leading to a deteriorated accuracy of WSSS. To alleviate this issue, we propose to adaptively partition the image content into deterministic regions (e.g., confident foreground and background) and uncertain regions (e.g., object boundaries and misclassified categories) for separate processing. For uncertain cues, we employ an activation-based masking strategy and seek to recover the local information with self-distilled knowledge. We further assume that the unmasked confident regions should be robust enough to preserve the global semantics. Building upon this, we introduce a complementary self-enhancement method that constrains the semantic consistency between these confident regions and an augmented image with the same class labels. Extensive experiments conducted on PASCAL VOC 2012 and MS COCO 2014 demonstrate that our proposed single-stage approach for WSSS not only outperforms state-of-the-art benchmarks remarkably but also surpasses multi-stage methodologies that trade complexity for accuracy. The code can be found at \url{https://github.com/Jessie459/feature-self-reinforcement}.

==> sections/conclusion.tex <==
\section{Conclusion}

In this work, we address the issue of reduced accuracy on object boundaries for the task of WSSS. This issue is rooted in the nature of the image-level supervised CAM, which only focuses on discriminative regions. Inspired by the observation that uncertain regions mainly cover ambiguous boundaries, we propose to estimate boundaries with the guidance of semantic uncertainty identified by CAM. To achieve this, we design an activation-based masking strategy and seek to recover local information with self-distilled knowledge. We further assume that the remaining unmasked regions should be robust enough to preserve global information. Based on this assumption, we introduce a self-distillation method to reinforce semantic consistency with another augmented view. We integrate our method into the single-stage WSSS framework and validate its effectiveness on PASCAL VOC 2012 and MS COCO 2014 benchmarks.

==> sections/experiments.tex <==
\section{Experiments}

\begin{table}[t]
    \centering
    \setlength{\tabcolsep}{1mm}
    \small{\begin{tabular}{l|c|c|cc}
        \toprule
        Method & Sup. & Net. & Val & Test \\
        \midrule
        \multicolumn{5}{l}{\textbf{\textit{Multi-stage WSSS methods}}.} \\
        RIB~\cite{lee2021reducing}  & $\mathcal{I}+\mathcal{S}$ & RN101 & 70.2 & 70.0 \\
        EDAM~\cite{wu2021embedded}  & $\mathcal{I}+\mathcal{S}$ & RN101 & 70.9 & 70.6 \\
        EPS~\cite{lee2021railroad}  & $\mathcal{I}+\mathcal{S}$ & RN101 & 71.0 & 71.8 \\
        SANCE~\cite{li2022towards}  & $\mathcal{I}+\mathcal{S}$ & RN101 & 72.0 & 72.9 \\
        L2G~\cite{jiang2022l2g}     & $\mathcal{I}+\mathcal{S}$ & RN101 & 72.1 & 71.7 \\
        RCA~\cite{zhou2022regional} & $\mathcal{I}+\mathcal{S}$ & RN38  & 72.2 & 72.8 \\
        SEAM~\cite{wang2020self}        & $\mathcal{I}$ & RN38  & 64.5 & 65.7 \\
        BES~\cite{chen2020weakly}       & $\mathcal{I}$ & RN101 & 65.7 & 66.6 \\
        CPN~\cite{zhang2021complementary}&$\mathcal{I}$ & RN38  & 67.8 & 68.5 \\
        CDA~\cite{su2021context}        & $\mathcal{I}$ & RN38  & 66.1 & 66.8 \\
        ReCAM~\cite{chen2022class}      & $\mathcal{I}$ & RN101 & 68.5 & 68.4 \\
        URN~\cite{li2022uncertainty}    & $\mathcal{I}$ & RN101 & 69.5 & 69.7 \\
        ESOL~\cite{li2022expansion}     & $\mathcal{I}$ & RN101 & 69.9 & 69.3 \\
        $\dagger$ViT-PCM~\cite{rossetti2022max}         & $\mathcal{I}$ & RN101 & 70.3 & 70.9 \\
        $\dagger$MCTformer~\cite{xu2022multi}           & $\mathcal{I}$ & RN38  & 71.9 & 71.6 \\
        $\dagger$OCR~\cite{cheng2023out}                & $\mathcal{I}$ & RN38  & 72.7 & 72.0 \\
        $\dagger$BECO~\cite{rong2023boundary}           & $\mathcal{I}$ & MiT-B2& 73.7 & 73.5 \\
        $\dagger$MCTformer+~\cite{xu2023mctformerplus}  & $\mathcal{I}$ & RN38  & 74.0 & 73.6 \\
        \midrule
        \multicolumn{5}{l}{\textbf{\textit{Single-stage WSSS methods}}.} \\
        RRM~\cite{zhang2020reliability}     & $\mathcal{I}$ & RN38  & 62.6 & 62.9 \\
        1Stage~\cite{araslanov2020single}   & $\mathcal{I}$ & RN38  & 62.7 & 64.3 \\
        $\dagger$AFA~\cite{ru2022learning}  & $\mathcal{I}$ & MiT-B1& 66.0 & 66.3 \\
        $\dagger$ToCo~\cite{ru2023token}    & $\mathcal{I}$ & ViT-B & 71.1 & 72.2 \\
        $\dagger$\textbf{Ours}        & $\mathcal{I}$ & ViT-B & \textbf{75.7} & \textbf{75.0} \\
        \bottomrule
    \end{tabular}}
    \caption{\small Performance comparison of semantic segmentation on PASCAL VOC 2012 in terms of mIoU(\%). Sup. denotes the supervision type. $\mathcal{I}$: image-level class labels. $\mathcal{S}$: off-the-shelf saliency maps. Net. denotes the segmentation network for multi-stage methods or the backbone for single-stage methods. RN38: Wide ResNet38~\cite{wu2019wider}, RN101: ResNet101~\cite{he2016deep}, MiT: Mix Transformer~\cite{xie2021segformer}. $\dagger$ denotes that the classification network or the backbone is based on Transformer.}
    \label{tab:sota_voc}
\end{table}

\begin{table}[t]
    \centering
    \small{\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l|c|c|c}
        \toprule
        Method & Sup. & Net. & Val \\
        \midrule
        \multicolumn{4}{l}{\textbf{\textit{Multi-stage WSSS methods}}.} \\
        EPS~\cite{lee2021railroad}      & $\mathcal{I}+\mathcal{S}$ & RN101 & 35.7 \\
        RIB~\cite{lee2021reducing}      & $\mathcal{I}+\mathcal{S}$ & RN101 & 43.8 \\
        L2G~\cite{jiang2022l2g}         & $\mathcal{I}+\mathcal{S}$ & RN101 & 44.2 \\
        CDA~\cite{su2021context}        & $\mathcal{I}$ & RN38  & 33.2 \\
        URN~\cite{li2022uncertainty}    & $\mathcal{I}$ & RN101 & 40.7 \\
        ESOL~\cite{li2022expansion}     & $\mathcal{I}$ & RN101 & 42.6 \\
        $\dagger$MCTformer~\cite{xu2022multi}           & $\mathcal{I}$ & RN38  & 42.0 \\
        $\dagger$ViT-PCM~\cite{rossetti2022max}         & $\mathcal{I}$ & RN101 & 45.0 \\
        $\dagger$OCR~\cite{cheng2023out}                & $\mathcal{I}$ & RN38  & 42.5 \\
        BECO~\cite{rong2023boundary}                    & $\mathcal{I}$ & RN101 & 45.1 \\
        $\dagger$MCTformer+~\cite{xu2023mctformerplus}  & $\mathcal{I}$ & RN38  & 45.2 \\
        \midrule
        \multicolumn{4}{l}{\textbf{\textit{Single-stage WSSS methods}}.} \\
        $\dagger$AFA~\cite{ru2022learning}  & $\mathcal{I}$ & MiT-B1    & 38.9 \\
        $\dagger$ToCo~\cite{ru2023token}    & $\mathcal{I}$ & ViT-B     & 42.3 \\
        $\dagger$\textbf{Ours}              & $\mathcal{I}$ & ViT-B     & \textbf{45.4} \\
        \bottomrule
    \end{tabular*}}
    \caption{\small Performance comparison of semantic segmentation on MS COCO 2014 in terms of mIoU(\%). We use the same notations as in Table~\ref{tab:sota_voc}.}
    \label{tab:sota_coco}
    \vspace{-5mm}
\end{table}

\subsection{Experimental Settings}

\subsubsection{Datasets.}
We evaluate our method on two benchmarks: PASCAL VOC 2012~\cite{everingham2010pascal} and MS COCO 2014~\cite{lin2014microsoft}. PASCAL VOC contains 20 object classes and one background class. Following the common practice of previous works~\cite{zhang2020reliability,araslanov2020single,ru2022learning,ru2023token}, it is augmented with data from the SBD dataset~\cite{hariharan2011semantic}, resulting in $10,582$, $1,449$ and $1,456$ images for training, validation and testing, respectively. MS COCO contains 80 object classes and one background class. It has $82,081$ images for training and $40,137$ images for validation. Note that we only adopt image-level labels during the training phase. We report mean Intersection-over-Union (mIoU) as the evaluation metric.

\subsubsection{Implementation Details.}
We adopt ViT-B~\cite{dosovitskiy2020image} pretrained on ImageNet~\cite{deng2009imagenet} as the transformer encoder. The convolutional decoder refers to DeepLab-LargeFOV~\cite{chen2017deeplab}. We use two aggregation blocks in the aggregation module. The projector comprises a 3-layer perceptron and a weight-normalized fully connected layer~\cite{caron2021emerging}. Parameters in the aggregation module and the projector are randomly initialized. We use a light data augmentation: random resized cropping to $448 \times 448$ with the scale $[0.32, 1.0]$ and the ratio $[3/4,4/3]$, random horizontal flipping, and random color jittering. The student network is optimized with AdamW~\cite{loshchilov2017decoupled}. The base learning rate is warmed up to $6e-5$ at the first 1,500 iterations and decayed with a polynomial scheduler. The weighting factors $(\lambda_1, \lambda_2, \lambda_3, \lambda_4, \lambda_5)$ are set to $(1.0,0.2,0.1,0.1,0.1)$. Particularly, $\lambda_4$ and $\lambda_5$ are decayed to $0.0$ with a cosine schedule. The teacher network requires no gradient and is updated with the EMA momentum. Experimentally, we find that synchronizing the teacher encoder with the student (i.e., momentum is $0.0$) works better. The momentum for the teacher projector is $0.996$ and increases to $1.0$ with a cosine schedule during training. We embrace the centering and sharpening technique suggested in~\cite{caron2021emerging} to avoid collapsed solutions. The masking ratio $r$ is $0.4$ for adaptive uncertain feature selection. The background scores $(\beta_l, \beta_h)$ introduced to determine uncertain areas are $(0.2,0.7)$. Training iterations are 20,000 for PASCAL VOC 2012 and 80,000 for MS COCO 2014. We use multi-scale testing and dense CRF~\cite{chen2014semantic} at test time following~\cite{ru2022learning,ru2023token}. 

\subsection{Comparison with State-of-the-arts}

\noindent \textbf{PASCAL VOC 2012.}
Table~\ref{tab:sota_voc} shows comparison results of our proposed Feature Self-Reinforcement (FSR) with other state-of-the-art methods on PASCAL VOC 2012. %Following the common practice~\cite{ru2022learning,ru2023token}, we report the final results of semantic segmentation with multi-scale testing and dense CRF processing. 
As can be seen from this table, FSR significantly outperforms other single-stage approaches, achieving $75.7\%$ and $75.0\%$ mIoU on the validation and test sets, respectively. It is noticeable that our method achieves even higher mIoU than several complicated multi-stage methods, e.g., FSR surpasses BECO~\cite{rong2023boundary} by margins of $2.0\%$ and $1.5\%$. Compared with multi-stage methods using both image-level labels and off-the-shelf saliency maps, e.g., L2G~\cite{jiang2022l2g} and RCA~\cite{zhou2022regional}, our method still achieves superior performance. We assume that although saliency maps are effective in providing additional background clues, our method can strengthen both deterministic areas (mostly the main body of objects or the background) and uncertain areas (mostly object boundaries), so that semantically distinct objects can be finely differentiated. Moreover, it can be seen that recent approaches with transformer-based networks (with $\dagger$) generally outperforms those with convolutional networks (without $\dagger)$. However, due to the difficulty of end-to-end optimization, single-stage transformer-based methods (e.g., ToCo reports $71.1\%$ and $72.2\%$) can only achieve comparable performance with multi-stage ones (e.g., BECO reports $73.7\%$ and $73.5\%$). Our method challenges this phenomenon and proves the effectiveness of transformer-based single-stage training. 

\noindent \textbf{MS COCO 2014.}
Table~\ref{tab:sota_coco} gives comparison results of semantic segmentation on a more challenging benchmark MS COCO 2014. We achieve $45.5\%$ mIoU on the validation set, which outperforms previous single-stage solutions and is slightly better than multi-stage MCTformer+~\cite{xu2023mctformerplus} by $0.2\%$. This further demonstrates the superiority of our proposed method. %Compared with AFA, CAMs generated by our method are more integral and confident. %For instance, 

\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/result.pdf}
    \caption{\small Visualization of WSSS attentions.}
    \label{fig:result}
    \vspace{-5mm}
\end{figure}

\noindent \textbf{Visualization Results.}
In Figure~\ref{fig:result}, we visualize CAMs derived from the classifier and semantic segmentation labels predicted by the decoder of three single-stage methods, i.e., AFA~\cite{ru2022learning}, ToCo~\cite{ru2023token} and our proposed FSR. Compared with AFA, ToCo and FSR can generate more integral and deterministic CAMs. For instance, the wheels of ``motorbike'' are mildly activated by AFA while strongly confirmed by ToCo and FSR. This proves the effectiveness of FSR for uncertain features. However, AFA only focuses on boosting uncertain features, whereas our method enhances both uncertain and certain ones. For instance, AFA mistakes ``drawer'' as ``chair'', while FSR successfully recognizes the different semantics. This shows the importance of FSR for deterministic features. 


\subsection{Ablation Studies}
In this section, we present extensive ablation studies to verify the effectiveness of our proposed FSR. We report the segmentation performance of the pseudo labels (Pseu.) derived from CAMs as well as the predicted segmentation labels (Pred.) generated by the decoder. All results are evaluated on the PASCAL VOC 2012 validation set. Multi-scale testing and dense CRF are not applied with ablation experiments. 

% \begin{figure}
%     \centering
%     \includegraphics[width=0.8\linewidth]{figures/masking_ratio.pdf}
%     \caption{\small Comparison results of the baseline, random token masking, absolute uncertain token masking and adaptive uncertain token masking w.r.t different masking ratios.}
%     \label{fig:masking_ratio}
% \end{figure}
\begin{table}[tbp]
    \centering
    \setlength{\tabcolsep}{1.5mm}
    % \small{\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}{c|c|c|ccccc}}
    \small{\begin{tabular}{c|c|c|ccccc}
        \toprule
        & Edge      & CAM       & \multicolumn{5}{c}{ CAM (masking ratio)} \\
        
        & (strict)  & (strict)  & 0.1 & 0.2 & 0.3 & 0.4 & 0.5  \\
        \midrule
        \multicolumn{8}{l}{\textit{Pseu. label results(\%)}} \\
        random      & -     & -     & 73.1          & 73.6          & \textbf{74.1} & 74.2          & 73.2          \\
        uncertain   & 73.3  & 74.0  & \textbf{74.1} & \textbf{74.2} & 73.9          & \textbf{74.4} & \textbf{73.7} \\
        \midrule
        \multicolumn{8}{l}{\textit{Pred. label results(\%)}} \\
        random      & -     & -     & 71.7          & 72.3          & 71.3          & 72.3          & 71.2          \\
        uncertain   & 71.6 & 71.8   & \textbf{72.2} & \textbf{72.3} & \textbf{72.0} & \textbf{72.5} & \textbf{72.1} \\
        \bottomrule
    \end{tabular}}
    \caption{\small Comparisons for uncertain feature selection methods. }
    \label{tab:uncertain_feature_selection}
   % \vspace{-5mm}
\end{table}

\subsubsection{Analyze of uncertain feature selection.}
Table~\ref{tab:uncertain_feature_selection} shows comparison results of uncertain feature selection methods. First, we compare two strict selection methods for uncertain features: edge-based selection and CAM-based selection. For edge-based selection, we choose the conventional Canny edge detector to extract structural edges in an image and generate exact masks of these edges. We set the activation thresholds for CAM-based selection to $(0.2,0.7)$. CAM-based selection is marginally better than edge-based selection. However, the improvement becomes considerable when CAM-based selection is relaxed, i.e., uncertain features are not strictly but preferentially masked. Empirically, we find that $r=0.4$ gives the best result. In addition, we can see that uncertain feature masking achieves higher performance than random feature masking in most cases. This demonstrates the importance of reinforcing uncertain features for semantics clarification.

% First, compared with the baseline that has no masking, applying \textit{absolute} uncertain token masking significantly improves segmentation performance from 67.9\% to 71.6\%. However, we argue that strictly masking uncertain tokens is not optimal as the uncertain tokens are filtered and determined by CAMs.......


% (1) verification of uncertain masking
% (2) verification of uncertain with random

\begin{table}[b]
    \centering
    % \begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}c|cc|cc}
    \small{\begin{tabular}{l|cc}
        \toprule
        Method & Pseu.(\%)   & Pred.(\%)  \\
        \midrule
        Baseline                    & 71.1 & 67.9 \\
        Baseline+unc.FSR            & 74.4 & 72.5 \\
        Baseline+unc.FSR+cer.FSR    & \textbf{75.7} & \textbf{73.6} \\
        % \midrule
        % \checkmark &            &            & 71.1 & 67.9 \\
        % \checkmark & \checkmark &            & 75.5 & 73.2 \\
        % \checkmark &            & \checkmark & 75.2 & 73.3 \\
        % \checkmark & \checkmark & \checkmark & \textbf{75.7} & \textbf{73.6} \\
        \bottomrule
    \end{tabular}}
    \caption{\small Ablations of feature self-reinforcement on uncertain areas (unc.FSR) and confident areas (cer.FSR). Pseu.: pseudo labels from CAMs. Pred.: predicted labels from the decoder.}
    \label{tab:ablation_TSD}
\end{table}

\subsubsection{Analyze of feature self-reinforcement.}
Table~\ref{tab:ablation_TSD} shows the ablation results of FSR on uncertain areas (unc.FSR) and on certain areas (cer.FSR). The masking ratio is set to $0.4$ for comparison.
% As mentioned in Section Methodology, our baseline is comprised of a transformer encoder and a convolutional decoder, supervised by the classification loss (i.e., $\mathcal{L}_{cls}$), the segmentation loss (i.e., $\mathcal{L}_{seg}$) and the affinity loss (i.e., $\mathcal{L}_{aff}$).
% It unfolds the advancement of the transformer-based architecture by achieving $71.7\%$ on pseudo labels and $67.9\%$ on predicted labels. However, there is an apparent performance gap when compared with well-designed multi-stage methods.
First, it demonstrates the advancement of unc.FSR by achieving $74.4\%$ (compared to $71.1\%$) on pseudo labels and $72.5\%$ (compared to $67.9\%$) on predicted labels. This proves that reinforcing uncertain features, which mainly contain ambiguous object boundaries and misclassified categories, is fairly effective. 
Second, when combining unc.FSR with cer.FSR, the quality of pseudo labels can be further improved, from $74.4\%$ to $75.7\%$. Consequently, predicted labels directly supervised by pseudo labels are promoted as well, from $72.5\%$ to $73.6\%$. This indicates that reinforcing deterministic features is complementary to unc.FSR with enhanced global understanding. 
% These results indicate that feature self-reinforcement on uncertain areas and on certain areas are both effective, as these strategies help enhance content understanding and semantic discrimination.
% Furthermore, we attain $75.7\%$ mIoU of pseudo labels and $73.6\%$ mIoU of predicted labels when combining unc.FSR and cer.FSR, demonstrating that these two strategies are complementary to each other. 

\begin{figure}[tbp]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/attention_entropy.pdf}
    \caption{\small Visualization of average attention entropy of different attention heads (dots) across different layers.}
    \label{fig:attention_entropy}
\end{figure}

\begin{figure}[tbp]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/CKA.pdf}
    \caption{\small Visualization of CKA similarity heatmaps between feature embeddings of patch tokens across different layers. The horizontal and vertical axes are layer indices.}
    \label{fig:CKA}
    \vspace{-5mm}
\end{figure}

% \begin{figure}[tbp]
%     \centering
%     \includegraphics[width=\linewidth]{figures/uncertain_TSD.pdf}
%     \caption{\small (a) Visualization of average attention entropy of different attention heads (dots) across different layers. (b) Visualization of CKA similarity heatmaps between feature embeddings of patch tokens across different layers.}
%     \label{fig:uncertain_TSD}
% \end{figure}

\noindent \textbf{(1) Analyze of unc.FSR.}
To gain an in-depth understanding of unc.FSR, we investigate the training process by analyzing \textit{attention maps} and \textit{feature maps}, and the visualization results are illustrated in Figure~\ref{fig:attention_entropy} and Figure~\ref{fig:CKA}.

For \textit{attention maps}, we compute average attention entropy~\cite{attanasio2022entropy} for each attention head across transformer layers. As can be seen from Figure~\ref{fig:attention_entropy} (a), attention entropy at shallow layers (e.g., layer 0 to 6) holds similar, however, it becomes higher and tighter at deep layers (e.g., layer 7 to 11) when unc.FSR is applied. Intuitively, a large entropy for a specific token indicates that a broad context contributes to this token, while a small entropy tells the opposite. From this point of view, we state that unc.FSR benefits semantic segmentation by improving the degree of contextualization at deep layers.

For \textit{feature maps}, we study similarities between feature embeddings of patch tokens across transformer layers via Centered Kernel Alignment (CKA)~\cite{nguyen2020wide}. Comparing the first row (w/o unc.FSR) and the second row (w/ unc.FSR) in Figure~\ref{fig:CKA} (b), we can find that CKA similarities become large with unc.FSR, especially at the beginning of the training process (e.g., $20\%$ and $40\%$). This indicates that representation structures of different layers become more related when unc.FSR is applied. The same pattern emerged with self-supervised learning is also reported in~\cite{xie2023revealing}. As the model reaches convergence, we can see that features at deep layers (e.g., layer 10) still resemble those at previous layers. This suggests that unc.FSR helps introduce low-level features, like edges and colors, to high-level abstract features, which is beneficial for pixel-level semantic segmentation.

\begin{table}[tbp]
    \centering
    \small{\begin{tabular}{c|cccc}
        \toprule
        & Baseline & GAP & GMP & MCA \\
        \midrule
        Pseu.(\%) & 71.1 & 72.3 & 71.8 & \textbf{75.2} \\
        Pred.(\%) & 67.9 & 70.9 & 70.0 & \textbf{73.3} \\
        \bottomrule
    \end{tabular}}
    \caption{\small Comparison of patch token aggregation methods. Pseu.: pseudo labels from CAMs. Pred.: predicted labels from the decoder.}
    \label{tab:aggregation}
\end{table}

\begin{figure}[tbp]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/class_attention.pdf}
    \caption{\small Visualization of class-to-patch attention maps derived from the aggregation module. Class labels are displayed below.}
    \label{fig:attention_maps}
    \vspace{-5mm}
\end{figure}

% \noindent \textbf{Analyze of certain feature aggregation.}
\noindent \textbf{(2) Analyze of cer.FSR}.
We compare the attentive aggregation of certain features with two intuitive methods: Global Average Pooling (GAP) and Global Maximum Pooling (GMP). Specifically, GAP assigns an equal weight to each unmasked patch token, while GMP picks up the dominant one along each dimension. As can be seen from Table~\ref{tab:aggregation}, GAP performs better than GMP. This is because GMP tends to intensify the most discriminative features, which may have an adverse effect in recognizing an integral object. The slight increase compared to the baseline may due to higher classification accuracy. It is noticeable that MCA outperforms GAP by a large margin, suggesting that an attentive weighting mechanism is superior to average weighting.
% To better understand the effect of the aggregation module, we illustrate class-to-patch attention maps in Figure~\ref{fig:attention_maps}. Note that the class token is not directly supervised by classification in our design. In fact, it interacts with unmasked patch tokens and learns to summarize effective information from them. 
To further demonstrate the effectiveness of masked cross-attention, we visualize class-to-patch attention maps in Figure~\ref{fig:attention_maps}. Note that the class token is not directly supervised by classification in our design. Actually, it interacts with unmasked patch tokens and learns to summarize effective information from them. This figure shows that the class token adaptively learns to pay attention to object regions. 

% Although GMP can only highlights the most discriminative features, it has been demonstrated that transformer-based classification networks benefit more from it~\cite{ru2022learning} due to the global modeling capability of self-attention. However, under the context of uncertainty-informed random masking, semantic integrity may be disturbed and GMP may become insufficient. In addition, GAP summaries information from each token uniformly and it is too straightforward to be optimal. To address these issues, we introduce an adaptive aggregation module that can attentively assign appropriate weights to different unmasked patch tokens.

==> sections/introduction.tex <==
\section{Introduction}

% Image segmentation is a fundamental and essential task that has extensive applications in computer vision. In the past, we have witnessed significant advances in a wide range of segmentation tasks such as semantic, instance and panoptic segmentation. For example, the recently released SAM~\cite{kirillov2023segment} has achieved a milestone due to its impressive zero-shot performance on downstream tasks. However, most success of these methods relies on a huge number of labor-intensive pixel-level annotations. To mitigate this issue, SAM~\cite{kirillov2023segment} designs an interactive data engine and build the SA-1B dataset with 1.1 billion segmentation masks.

% Another line of work is Weakly Supervised Semantic Segmentation (WSSS) that 
Weakly Supervised Semantic Segmentation (WSSS) aims at cutting the budget of annotating `strong" pixel-level labels by using `weak" labels such as bounding boxes~\cite{dai2015boxsup,song2019box}, scribbles~\cite{lin2016scribblesup,vernaza2017learning}, points~\cite{bearman2016s, su2022sasformer} and image-level class labels~\cite{araslanov2020single, zhang2021weakly, ru2022learning,ru2023token}. This paper focuses on WSSS with the supervision of image-level class labels that are the most affordable yet challenging among WSSS scenarios. 

\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/teaser.pdf}
    % \caption{\small (a) shows an image with its ground truth. (b) illustrates the corresponding CAM, which identifies the most discriminative areas, e.g., the main body of a person/horse. (c) shows the pseudo label derived from the CAM. We propose to improve the pseudo label with two motivations. First, non-discriminative areas should understand its own content, e.g., is a horse leg or background. Second, discriminative areas should be reinforced to have more precise meanings, e.g., person and horse are semantically distinct.}
    \caption{\small Illustration of our main idea. The flawed CAM only identifies discriminative regions. To mitigate this issue, we propose to partition the image into uncertain regions (e.g., object boundaries) and confident regions (e.g., the main body of an object) and reinforce features of these regions in a complementary way.}
    \label{fig:teaser}
    \vspace{-5mm}
\end{figure}

Existing methods commonly train a classification network with class labels and then generate Class Activation Maps (CAMs)~\cite{zhou2016learning} as seed regions. CAMs are further refined to pseudo segmentation labels, which are treated as Ground Truth (GT) for supervising a segmentation network.
These steps can be processed in separate stages or collaborated in one stage. Particularly, the single-stage framework is more efficient as it streamlines the training pipeline. Whatever the case is, one common belief is that high-quality pseudo labels generally lead to superior semantic segmentation performance. Consequently, we focus on seeking solutions for obtaining accurate pseudo labels within the single-stage framework. 

However, CAMs are essentially flawed because they are intended for classification, i.e., they strive to identify the most discriminative regions of an object for improved classification accuracy. To tackle this issue, several methods are proposed to improve the initial seeds~\cite{li2018tell,hou2018self,jiang2019integral,lee2019ficklenet,wang2020self,lee2021reducing, he2023mitigating} or refining pseudo labels~\cite{ahn2018learning,ahn2019weakly,chen2020weakly} by growing activations or labels to semantically consistent pixels in the neighborhood.
Some recent studies find the restricted receptive field of convolution has a negative impact on recognizing whole objects~\cite{ru2022learning,ru2023token}. Thus, they build solutions on Vision Transformer (ViT)~\cite{dosovitskiy2020image} to model global relationships for the task. Despite the global modeling capability, we argue that the issue of CAM seeds or pseudo labels is not explicitly resolved.
We experimentally observe that uncertain regions mainly contain \textbf{\textit{boundary regions between the foreground objects and the background}}, and \textbf{\textit{misclassified regions within multiple semantically-different objects}}. Taking an example from Figure~\ref{fig:teaser}, the generated CAM is uncertain about the two arms of the ``person" on the ``chair", and the boundary between the foreground (``person" and ``chair") and the background is unclear. These uncertain regions are easily confused by obscure semantic clues because pixel-level supervision is totally absent. 

Our goal in this work is to clarify the visual semantics of uncertain regions covered by the uncertain regions mentioned above. To achieve this, we figure that the local visual patterns should be explicitly modeled and captured. As can be seen from Figure~\ref{fig:teaser}, \textit{the head} and \textit{upper thighs} are well recognized, while \textit{arms} and \textit{lower legs} need to be promoted. A classification network should be enhanced with local contexts so that it can understand that \textit{arms and lower legs surely belong to a person}. 
% There are two intuitions to achieve this goal. First, the local visual patterns over uncertain regions should be explicitly perceived and captured. For example, the legs of a horse should be labeled as \texttt{horse}, not \texttt{background}, and the legs of a person should be labeled as \texttt{person}, not \texttt{horse}. Second, the global semantic meanings over discriminative regions should stay consistent with the original image so that pixels in non-discriminative regions can have a clear target to approach. For example, the bodies of a horse and a person should be robustly separable to ease the classification of legs. 
Note that some methods in the literature deal with noisy object boundaries by employing an off-the-shelf saliency detection model for rich object contours~\cite{lee2021railroad,li2022towards}, which overlook the uncertain regions caused by low confidence in foreground objects. %Nevertheless, we believe there is no need to introduce an extra model trained for an extra stage as pre-processing. 
Instead, the training objective can be attained from the knowledge of past training iterations, i.e., self-distillation~\cite{caron2021emerging}. Following this philosophy, we discard any saliency detection model and take advantage of the potential of self-distillation to form our training objectives. 

To this end, we propose a progressive self-reinforcement method to explore and strengthen semantics over uncertain regions. To distinguish uncertain pixels from confident pixels, we define pixels with moderate CAM scores as uncertain pixels, since a very low/high score strongly indicates the background/foreground. Specifically, we propose to mask corresponding uncertain features and learn to recover the original information with the help of an online momentum teacher. 
% Specifically, we propose two complementary modules to facilitate latent semantic layouts of images. One module is devised to mask corresponding uncertain patch tokens and try to recover information with the help of an online momentum teacher.
This module aligns with Masked Image Modeling (MIM), a popular pretraining paradigm that brings locality inductive bias to the model~\cite{xie2023revealing}. We upgrade its random masking strategy with semantic uncertainty so that the network can focus on uncertain features controlled by the masking ratio. This module is beneficial to facilitate features in both object boundaries and misclassified regions. 
% Masked patch tokens with vague semantics progressively learn to reconstruct probability distributions with the knowledge from the self-distilled teacher. As a result, uncertain tokens gradually get close to semantically related confident tokens in the feature space, which is beneficial for clarifying object boundaries.
We further assume that the corresponding confident features should be robust enough to present global semantics. Based on this assumption, we introduce a complementary method that constrains semantic consistency between the current and augmented views with the same class labels. Our method can be seamlessly integrated into the vision transformer based single-stage WSSS framework. 
% The other module is devised to bootstrap representations of the remaining visible patch tokens so that masked tokens can have a determined target to get close to. This is achieved by enforcing a similarity between the visible signal from one distorted view and the overall signal from another distorted view. We believe that discriminative regions should adequately represent the original image, and this regularization technique is helpful in distinguishing different categories of objects, including the background. 


In summary, our main contributions are as follows:
\begin{itemize}
    \item We propose a novel approach known as progressive uncertain feature self-reinforcement, aiming to enhance the semantics of uncertain regions effectively. The investigation of the uncertain region, which involves object boundaries and misclassified categories, improves the performance of WSSS significantly.
    % We introduce self-distillation to reinforce uncertain features to clarify ambiguous boundaries and misclassified labels.
    % \item We propose a progressive uncertain feature self-reinforcement method for WSSS. Unlike previous mainstream works that adopt an extra saliency detection model trained for an extra stage, we locate regions of uncertainty with the help of CAMs generated from the classifier within the same training pipeline.
    \item We design an adaptive masking strategy to determine uncertain features. Unlike previous mainstream studies that adopt an additional saliency detection model, we locate uncertain regions with the guidance of semantic-aware CAMs.
    % \item We propose token self-distillation to explore semantics over uncertain regions and strengthen semantics over confident regions. Consequently, deterministic features and uncertain features can be constrained to possess the correct semantics. 
    \item Exhaustive experiments on PASCAL VOC 2012~\cite{everingham2010pascal} and MS COCO 2014~\cite{lin2014microsoft} show that our method outperforms SOTA single-stage competitors, even better than existing complicated multi-stage methods. 
\end{itemize}

% 1. 图像分割作为视觉经典任务，在xxx 诸多场景有广泛用处。近年来，随着深度学习技术的不断变革，语义分割、实例分割、全景分割等方法均取得了较大的进步，尤其是近期的SAM模型，取得了里程碑式的分割成效。然而，这些方法较好的成果大多依赖大量精细的像素级标签，像素级标签的标注通常是十分耗时、耗力的。

% 2. 为了有效应对大量标注的不足，诸多提出了弱监督的图像分割方法。 通过利用类别、点、框、部分标注等弱监督形式，实现图像的精细分割。xxxx 介绍下当前弱监督的图像分割方法（按照类型简单介绍）。

% 3. 当前的弱监督方法取得了不错的成效，但距离全监督分割仍有一定的差距。主要的挑战在于，物体边缘、类似背景等难分割区域的难以有效、精准分割。

% 4. 为了有效上述 不确定区域的精准分割挑战，本文聚焦于弱监督的语义分割任务，提出了xxxx方法。


==> sections/method.tex <==
\section{Methodology}

% Due to the fact that only image-level classification labels are given to perform the task of pixel-level semantic segmentation, the predicted results are usually vulnerable to inaccuracy on semantic boundaries, either failing in recognizing complete object areas or containing unexpected background. Inspired by the favorable property that vision transformer trained in a self-supervised manner automatically contains object boundaries within its features~\cite{caron2021emerging}, we introduce Patch-Token Self-Distillation (PTSD) to help enhance object boundaries so that the overall segmentation performance can be further promoted. Specifically, we propose to perform \textit{PTSD on uncertain regions} to comprehend the semantic layout of object boundaries. Based on the intuition that one object should be well recognized by its discriminative features, we further propose to conduct \textit{PTSD on confident regions} to further escalate localization of foreground objects.

\subsection{Single-Stage Framework for WSSS}
Our single-stage framework for WSSS is illustrated in Figure~\ref{fig:overview}. We embrace an encoder-decoder architecture to accomplish semantic segmentation with image-level supervision. The encoder is a vision transformer supervised by class labels. Besides, we adopt Patch Token Contrast (PTC) proposed in~\cite{ru2023token} for affinity learning as it is crucial to constrain affinities between patch tokens of the last layer against over-smoothing~\cite{gong2021vision}. As for semantic segmentation, we borrow a lightweight convolutional decoder from DeepLab~\cite{chen2017deeplab}, which is supervised by reliable pseudo segmentation labels that are generated from CAMs. In addition, we use an aggregation module to summarize part of patch tokens into one class token and an MLP-based projector to transform all tokens into an appropriate feature space for feature learning. To achieve self-distillation, we introduce the aggregation module, the projector, and the teacher network that shares the same backbone with the transformer encoder. 

Formally, let $\mathcal{F}$ be the encoder, $\mathcal{P}$ be the projector, $\mathcal{M}$ be the masking operator, and $\mathcal{A}$ be the aggregating operator, we formulate the pipeline as follows. First, an input image is randomly augmented to two distorted views: $x_1$ and $x_2$. Each view is subsequently divided into $HW$ non-overlapping patch tokens, denoted as $T_1=\{t_1^{(i)}\}_{i=1}^{HW}$ and $T_2=\{t_2^{(i)}\}_{i=1}^{HW}$, respectively. Taking the student pipeline as an example, we assume that $T_1$ is for classification while $T_2$ is for feature reinforcement. For classification, $T_1$ is fed into the encoder to obtain classification logits, i.e., $Z_1=\mathcal{F}(T_1)$. For feature reinforcement, we separate $T_2$ into uncertain and certain tokens and only mask uncertain tokens. The resulting masked view, denoted as $\hat{T}_2=\mathcal{M}(T_2)$, is forwarded through the encoder as well, i.e., $\hat{Z}_2=\mathcal{F}(\hat{T}_2)$. Next, $\hat{Z}_2$ is fed into the aggregation module in which unmasked tokens are summarized into one class token. The output class token is concatenated with the input patch tokens, then they are projected and normalized to probability distributions:
\begin{equation}
    \hat{P}_2 = \sigma\left( \mathcal{P}\left( [\mathcal{A}\left(\hat{Z}_2\right);\hat{Z}_2 ] \right) \right) 
\end{equation}
where $\sigma$ is the softmax function and $[;]$ represents concatenation. The teacher pipeline is similar to the student pipeline, except that $T_1$ and $T_2$ are both non-masked, and we finally obtain two distributions $P_1$ and $P_2$. 

\subsection{Uncertain Feature Selection}
We first briefly introduce how to generate CAMs, then elaborate on how to select uncertain features of patch tokens with the guidance of semantic-aware CAMs.

We feed the input image into the transformer encoder for CAM generation and obtain $Z \in \mathbb{R}^{HW \times D}$, where $D$ is the embedding dimension. The CAM is generated by linearly projecting $Z$ with the classifier weights $W \in \mathbb{R}^{C \times D}$, where $C$ is the number of classes. The normalized CAM, denoted as $M_c \in \mathbb{R}^{HW \times C} (0 \leq M_C \leq 1)$, is attained with the $\operatorname{ReLU}$ function and $\operatorname{min-max}$ normalization:
\begin{equation}
    M_c := \operatorname{min-max}(\operatorname{ReLU}(ZW^{\top}))
\end{equation}
%A background score $\beta \in (0, 1)$ is manually set to differentiate the background from foreground objects.

% We adopt patch-aligned masking strategy~\cite{bao2021beit,he2022masked,xie2022simmim} since it is convenient and efficient to operate on the basic processing unit of vision transformer. As described in Sec. Preliminaries, we divide an input image into $(H_i / P) \times (W_i / P)$ non-overlapping patches. Given the mask patch size $P_m$, which is a multiple of $P$, we aim to construct a $(H_i / P_m) \times (W_i / P_m)$ mask that indicates which groups of patches are kept or masked. The constructed mask is then scaled up and applied to patch tokens before feeding them into any transformer block. In practice, we use a learnable mask token to replace masked patch tokens~\cite{xie2022simmim}.

To determine uncertain features of patch tokens, we first identify uncertain areas of the generated CAM, then conduct an adaptive masking strategy where uncertain patches are given priority to be masked. Inspired by~\cite{zhang2020reliability,ru2022learning}, we introduce two background thresholds $\beta_l$ and $\beta_h$ ($0 < \beta_l < \beta_h < 1$) to partition the $M_c$ into reliable and non-reliable areas. We regard features in non-reliable areas as uncertain features. However, some reliable areas may be wrongly labeled, and features in these areas should also be considered uncertain. To remedy this issue, we propose an adaptive masking strategy where masking is flexibly guided by semantic uncertainty. Specifically, we introduce a refined $M_s \in \mathbb{R}^{HW}$.
%where each element is initially sampled from the standard uniform distribution $U(0,1)$. 
%This sampling matrix is then injected with semantic uncertainty in a piecewise manner:
\begin{equation}
    M_s=\left\{
    \begin{array}{lr}
    u_i+1, & \text{if } \beta_l < \max (M_c^{(i,:)}) < \beta_h \\
    u_i, & \text{otherwise}
    \end{array}\right.
\end{equation}

where $u_i \sim U(0,1)$. The rationale behind this lies in its utilization as a means to operationalize an uncertain ratio $r \in (0,1)$ functioning as a hyperparameter for regulating proportions. To elaborate, when the uncertain region defined by $r$ resides within the confines of the salient region as determined by the CAM (e.g., $\beta_l < \max (M_c^{(i,:)}) < \beta_h$), the allocation of the uncertain region is stochastically determined through the employment of $u_i$. Conversely, in cases where the uncertain region stipulated by $r$ surpasses the boundaries of the CAM's saliency region, the surplus region is subjected to random allocation.

\begin{equation}
    M_b^{(i)}=\left\{
    \begin{array}{lr}
    1, & \text{if } i \in \argtopk(M_s), k:= \lfloor HW * r \rfloor \\
    0, & \text{otherwise}
    \end{array}\right.  
\end{equation}

We select uncertain tokens in $M_s$ using the uncertainty ratio $r$, where $\lfloor \rfloor$ represents the floor function. Each element in $M_b$ with a value of 1 indicates that the corresponding floating value in $M_s$ falls within the lower $r$ proportion of the overall ranking; a value of 0 indicates that it falls outside the $r$ proportion.
% We repeatedly mask the token with the highest value in the sampling matrix until a predefined masking ratio $r \in (0,1)$ is reached.
% Here we introduce a binary mask $M_b=\{0,1\}^{HW}$ where masked positions are 1 and unmasked positions are 0. 

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/MCA.pdf}
    \caption{\small Illustration of the aggregation module. This module is composed of several aggregation blocks, where each block alternates in turn a cross-attention layer and a feed-forward layer. The cross-attention layer computes attention between a class token and a sequence of unmasked patch tokens.}
    \label{fig:aggregation}
\end{figure}

\subsection{Certain Feature Aggregation}
We design an attentive aggregation module to compress a sequence of patch tokens $\hat{Z} \in \mathbb{R}^{HW \times D}$ into one class token $\bar{Z} \in \mathbb{R}^{1 \times D}$. As shown in Figure~\ref{fig:aggregation}, this module is composed of several aggregation blocks, where each block contains a Masked Cross-Attention (MCA) layer and a Feed-Forward (FF) layer:
\begin{equation}
    \begin{aligned}
    \bar{Z}^{(l)} & =\bar{Z}^{(l)}+\text{MCA}\left(\eta([\bar{Z}^{(l)};\hat{Z}^{(l)}])\right) \\
    \bar{Z}^{(l+1)} & =\bar{Z}^{(l)}+\text{FF}\left(\eta(\bar{Z}^{(l)})\right)
    \end{aligned}
\end{equation}
where $l$ denotes the layer index and $\eta$ is the LayerNorm~\cite{ba2016layer}.

MCA is analogous to self-attention~\cite{vaswani2017attention}, except that it computes attention between the class token and a set of unmasked patch tokens. We parameterize MCA with projection weights $W_Q,W_K,W_V,W_O \in \mathbb{R}^{D \times D}$. Queries $Q \in \mathbb{R}^{1 \times D}$, keys $K \in \mathbb{R}^{HW \times D}$ and values $V \in \mathbb{R}^{HW \times D}$ are calculated as:
\begin{equation}
    Q = W_Q \eta\left( \bar{Z} \right), K = W_K \eta\left( \hat{Z} \right), V = W_V \eta\left( \hat{Z} \right)
\end{equation}
Note that queries are derived from the class token, while keys and values are calculated on patch tokens. The masked cross-attention $A \in \mathbb{R}^{1 \times HW}$ is formulated as follows:
\begin{equation}
    A = \sigma \left( \frac{\left(1-M_b\right) \left( QK^{\top} \right)}{\sqrt{D}} \right)
\end{equation}
The output of MCA is computed as a weighted sum of values, i.e., $W_O\left(AV\right)$.
% The cross-attention based aggregation can be considered as a compromise between GAP and GMP. On the one hand, GAP might become deficient if the size of the object is too small or there are too many background regions. On the other hand, GMP might become inadequate if the size of the object is too large or there are a number of objects. Our aggregation approach can mitigate these issues by paying attention to discriminative patches in a learnable way.

\subsection{Feature Self-reinforcement}
We adopt self-distillation~\cite{caron2021emerging,zhou2021ibot,oquab2023dinov2} in the literature to supervise the learning process of feature reinforcement. As mentioned at the beginning of this section, given two distorted views of the same image, we compute one student output $\hat{P}_2$ and two teacher outputs $P_1$ and $P_2$. To be specific, the self-reinforcement loss for uncertain features $\mathcal{L}_{u}$ is an average of the cross-entropy loss between a masked student patch token and its corresponding teacher patch token:
\begin{equation}
    \mathcal{L}_{u} = -\sum_{i=1}^{HW} M_b^{(i)} P_2[1:]^{(i)} \log \hat{P}_2[1:]^{(i)}
\end{equation}
Here $M_b$ is the mask mentioned above to help select masked patch tokens. The reinforcement loss for certain features $\mathcal{L}_{c}$ is the cross-entropy loss calculated on two cross-view class tokens:
\begin{equation}
    \mathcal{L}_{c} = -P_1[0] \log \hat{P}_2[0]
\end{equation}

Following the common practice, we adopt the multi-label soft margin loss $\mathcal{L}_{cls}$ for classification learning, the pixel-wise cross-entropy loss $\mathcal{L}_{seg}$ for segmentation learning, and the cosine similarity loss $\mathcal{L}_{aff}$ for affinity learning. Given weighting factors $\lambda_{*}$, the overall training objective is:
\begin{equation}
    \begin{split}
    \mathcal{L} = \lambda_{1} \mathcal{L}_{cls} + \lambda_{2} \mathcal{L}_{aff} + \lambda_{3} \mathcal{L}_{seg} 
    +\lambda_{4} \mathcal{L}_{u} + \lambda_{5} \mathcal{L}_{c}
    \end{split}
\end{equation}

% \noindent \textbf{Uncertain Token Self-Distillation.}
% We perform our proposed masking strategy to the augmented input image $x$ and obtain its masked view $\hat{x}$. The student network takes the masked view $\hat{x}$ and outputs projection embeddings $\mathbf{P}_s(\hat{x})$, while the teacher network takes the non-masked image $x$ and outputs projection embeddings $\mathbf{P}_t(x)$. The training objective is formulated as follows:
% \begin{equation}
%     \mathcal{L}_u = -\sum_{i=1}^{HW} \mathbf{m}^{(i)} \mathbf{P}_t(x)^{(i)} \log \mathbf{P}_s(\hat{x})^{(i)}
% \end{equation}
% Here $\mathbf{m} \in [0, 1]^{HW}$ denotes a binary mask where $1$ means being masked and $0$ means being kept.

% \noindent \textbf{Confident Token Self-Distillation.}
% There are two intuitive options that can be chosen to aggregate a set of unmasked token embeddings: global average pooling (GAP) and global max pooling (GMP). Although GMP can only highlights the most discriminative features, it has been demonstrated that transformer-based classification networks benefit more from it~\cite{ru2022learning} due to the global modeling capability of self-attention. However, under the context of uncertainty-informed random masking, semantic integrity may be disturbed and GMP may become insufficient. In addition, GAP summaries information from each token uniformly and it is too straightforward to be optimal. To address these issues, we introduce an adaptive aggregation module that can attentively assign appropriate weights to different unmasked patch tokens.


% % \subsubsection{Training Objective of Confident Regions.}
% First, we construct two augmented views $x_1$ and $\hat{x}_2$ from the same input image. The first view $x_1$ is fully visible and is forwarded through both the encoder and the decoder to perform end-to-end semantic segmentation. The second view $\hat{x}_2$ is partially masked according to our proposed masking strategy. Next, $x_1$ is fed into the teacher encoder $\mathcal{E}_t$ and the teacher aggregation module $\mathcal{A}_t$ to obtain the teacher class embedding $\bar{t}_t$. The student class embedding $\bar{t}_s$ is attained via the same procedure with the student network:
% \begin{equation}
%     \begin{aligned}
%     \bar{t}_t &= \mathcal{A}_t(\mathcal{E}_t(x_1)) \\
%     \bar{t}_s &= \mathcal{A}_s(\mathcal{E}_s(\hat{x}_2)) \\
%     \end{aligned}
% \end{equation}
% The training objective is to minimize the cross-entropy loss between projected class embeddings:
% \begin{equation}
%     \mathcal{L}_c = -\mathbf{P}_t(\bar{t}_t) \log \mathbf{P}_s(\bar{t}_s)
% \end{equation}
% Following DINO~\cite{caron2021emerging}, we avoid model collapse by centering and sharpening of the output of the momentum teacher.

==> sections/preliminary.tex <==
\section{Preliminaries} \label{sec:preliminaries}

In this section, we introduce the fundamental knowledge of CAM generation, vision transformer and knowledge distillation in brief.

\noindent \textbf{CAM Generation.}
Class Activation Maps (CAM)~\cite{zhou2016learning} have been widely adopted to generate pseudo segmentation labels for WSSS. Concretely, given an input image and its extracted features $\mathbf{F}  \in \mathbb{R}^{D \times HW}$ with an encoder network (e.g., ViT), where $D$ is the channel dimension and $HW$ is the spatial dimension, we compute the raw CAM $\mathbf{M}^{\prime} \in \mathbb{R}^{C \times HW}$ by linearly projecting the features with the weights $\mathbf{W} \in \mathbb{R}^{C \times D}$ in the classification layer, where $C$ is the number of object categories. The normalized CAM $\mathbf{M} \in \mathbb{R}^{C \times HW}$ is then obtained by applying $\mathtt{ReLU}$ function and $\mathtt{MinMax}$ normalization. The above mentioned process can be formulated as:
\begin{equation}
    \mathbf{M}^{\prime} = \mathbf{W} \mathbf{F},
    \mathbf{M} = \mathtt{MinMax}(\mathtt{ReLU}(\mathbf{M}^{\prime}))
\end{equation}
A background threshold $\beta \in (0, 1)$ is manually assigned to differentiate background from foreground objects.

\noindent \textbf{Vision Transformer.}
We use the standard vision transformer as the encoder network. An input image with spatial dimensions $H_i \times W_i$ is first split into $H \times W$ patches, then these patches are projected and flattened to form a sequence of patch tokens $\{t^{(i)}\}_{i=1}^{HW}$. Here $H = H_i / P$ and $W = W_i / P$, $P$ is the patch size. Note that we ignore the class token as it is not used for classification. Next, the transformer block alternates self-attention (SA) layers with feed-forward (FF) layers:
\begin{equation}
    \begin{aligned}
    t_{l}^{\prime} &=t_{l}+\operatorname{SA}\left(\mathcal{N}\left(t_{l}\right)\right) \\
    t_{l+1} &=t_{l}^{\prime}+\operatorname{FF}\left(\mathcal{N}\left(t_{l}^{\prime}\right)\right)
    \end{aligned}
\end{equation}
where $l$ is the layer index and $\mathcal{N}$ is LayerNorm~\cite{ba2016layer}. After forwarding through transformer blocks, the encoded sequence of patch tokens is fed into a fully-connected layer to perform classification.

\noindent \textbf{Self-Distillation.}
Self-distillation~\cite{caron2021emerging,zhou2021ibot,oquab2023dinov2} distills knowledge from a teacher network $\mathcal{F}_t$ to a student network $\mathcal{F}_s$, where the teacher and the student share the same architecture, consisting of an encoder $\mathcal{E}$ and a projection head $\mathcal{H}$. Particularly, teacher parameters $\theta_t$ are updated via Exponential Moving Average (EMA) of student parameters $\theta_s$. Taking the student network for example, given an input image $x$, the probability distribution $\mathbf{P}_s$ over $K$ dimensions is calculated by normalizing the output of the network with a $\texttt{softmax}$ function:
\begin{equation}
    \mathbf{P}_s(x)^{(i)} = \frac{\exp(\mathcal{F}_s(x)^{(i)} / \tau_s)}{\sum_{k=1}^{K}\exp (\mathcal{F}_s(x)^{(k)} / \tau_s)}
\end{equation}
where $\tau_s$ is a temperature parameter that controls the shape of the distribution. We can formulate $\mathbf{P}_t$ with temperature $\tau_t$ in the same way. Knowledge is therefore distilled from the teacher network to the student network by minimizing the cross-entropy loss over these two distributions:
\begin{equation}
    \mathcal{L} = -\mathbf{P}_t(x_1) \log \mathbf{P}_s(x_2)
\end{equation}
Here $x_1$ and $x_2$ represent two distorted views of the same image $x$ via random augmentations, following the common practice in self-supervised learning~\cite{chen2020simple,grill2020bootstrap,chen2021exploring}.


==> sections/related_work.tex <==
\section{Related Work}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/overview.pdf}
    \caption{\small Overview of our framework. For the student pipeline, we forward one view through the encoder, and the encoded patch tokens are fed into the classifier for classification and the decoder for semantic segmentation, separately. The other view is masked and sequentially forwarded through the encoder, the aggregation module, and the projector. For the teacher pipeline, both views are propagated through the encoder, the aggregation module, and the projector. The teacher network requires no gradient and is an exponential moving average (EMA) of the student network.}
    \label{fig:overview}
\end{figure*}

% 2023 papers
% Token contrast for weakly-supervised semantic segmentation, CVPR 2023
% Out-of-candidate rectification for weakly supervised semantic segmentation, CVPR 2023
% Clip is also an efficient segmenter: A text-driven approach for weakly supervised semantic segmentation
% Sparse Multimodal vision transformer for Weakly Supervised Semantic Segmentation
% Weakly Supervised Semantic Segmentation via Adversarial Learning of Classifier and Reconstructor
% Weakly-supervised semantic segmentation via online pseudo-mask correcting
% Segment Anything is A Good Pseudo-label Generator for Weakly Supervised Semantic Segmentation
% Boundary-Enhanced Co-Training for Weakly Supervised Semantic Segmentation
% Self Correspondence Distillation for End-to-End Weakly-Supervised Semantic Segmentation

\subsection{Weakly Supervised Semantic Segmentation}
\noindent \textbf{Multi-stage WSSS methods} commonly adopt a classification network to generate CAMs as pseudo labels, then train a segmentation network for evaluating the final performance. To overcome the well-known weakness that CAM only focuses on discriminative areas, several previous works try to improve the training dynamic by erasing and seeking~\cite{hou2018self,li2018tell}, introducing adversarial learning~\cite{lee2021anti,yoon2022adversarial} or self-supervised learning~\cite{shimoda2019self,chen2022self}. Recent approaches also adopt vision transformer~\cite{dosovitskiy2020image} to perform WSSS, considering its favorable long-range modeling capability. TS-CAM~\cite{gao2021ts} proposes to couple class-agnostic attention maps with semantic-aware patch tokens to promote object localization. MCTformer~\cite{xu2022multi} introduces multiple class tokens so that class-specific attention maps can be generated. Other methods incorporate extra data into training or post-processing, e.g., saliency maps~\cite{lee2021railroad,wu2021embedded} or Contrastive Language-Image Pre-training (CLIP) models~\cite{xie2022clims,lin2023clip}. Our solution aims at improving pseudo labels as well, but it is integrated into a single-stage framework for simplicity, and it requires neither extra data nor off-the-shelf models. 

% ~\cite{wei2017object,kumar2017hide,hou2018self}, 
% that are either applied on images~\cite{li2018tell,zhang2021complementary,yoon2022adversarial} or feature maps~\cite{hou2018self,lee2019ficklenet,chen2022class}.

% Other methods incorporate cross-image information~\cite{sun2020mining,li2021group}, contrastive learning~\cite{ke2021universal,du2022weakly,zhou2022regional} and self-supervised learning~\cite{shimoda2019self,wang2020self,chen2022self} to enhance the quality of CAMs.

\noindent \textbf{Single-stage WSSS methods} generally treat multiple stages such as classification, pseudo label refinement, segmentation as a whole and perform joint training. 1Stage~\cite{araslanov2020single} achieves comparable performance with prevailing multi-stage models by ensuring local consistency, semantic fidelity and mask completeness. AFA~\cite{ru2022learning} explores the intrinsic architecture of vision transformer and derives reliable semantic affinity from multi-head self-attention for pseudo label refinement. ToCo~\cite{ru2023token} tackles the issue of over-smoothing observed in vision transformer by supervising the final patch tokens with intermediate knowledge. Despite the simplified and streamlined training procedure, single-stage methods often suffer from inferior performance when compared with multi-stage ones. In this work, we achieve superior semantic segmentation results with the single-stage framework by discovering and reinforcing underlying semantic layouts. 

% \subsection{vision transformer for WSSS.}
% vision transformer~\cite{dosovitskiy2020image} has achieved great success in various vision tasks, including WSSS~\cite{gao2021ts, xu2022multi, ru2022learning, ru2023token}. TS-CAM~\cite{gao2021ts} proposes to couple class-agnostic attention maps with semantic-aware patch tokens to advance object localization. MCTformer~\cite{xu2022multi} introduces multiple class tokens so that ViT can exploit class-specific attention maps. AFA~\cite{ru2022learning} explores the inherent virtue of ViT and derives reliable semantic affinity from self-attention to refine pseudo labels. ToCo~\cite{ru2023token} tackles the issue of over-smoothing observed in vision transformer by supervising the final patch tokens with intermediate knowledge. 

\subsection{Self-Distillation}
Self-distillation associates self-supervised learning~\cite{chen2020simple,he2020momentum,grill2020bootstrap,chen2021exploring} with knowledge distillation~\cite{hinton2015distilling}, where knowledge is transferred and learned without resorting to any labels. It is primarily designed to compress large networks and hopefully promote performance on downstream tasks via mimicking the output of a frozen teacher~\cite{noroozi2018boosting,passalis2020heterogeneous,fang2021seed,chen2022knowledge}. Recently, some works~\cite{caron2021emerging,zhou2021ibot} build the teacher dynamically during training, where the teacher adopts the same architecture as that of the student and is updated with the knowledge of past iterations. The resulting framework simplifies the training process and achieves compelling results when compared with other self-training frameworks. We follow the basic idea of self-distillation and adapt it to the task of WSSS for the purpose of exploring inaccurate object boundaries as well as improving discriminative object features. 

